LLM NL2SQL Robustness: Surface Noise vs. Linguistic Variation in Traditional and Agentic Settings

Robustness evaluation for Natural Language to SQL (NL2SQL) systems is essential because real-world database environments are dynamic, noisy, and continuously evolving, whereas conventional benchmark evaluations typically assume static schemas and well-formed user inputs. In this work, we introduce a robustness evaluation benchmark containing approximately ten types of perturbations and conduct evaluations under both traditional and agentic settings. We assess multiple state-of-the-art large language models (LLMs), including Grok-4.1, Gemini-3-Pro, Claude-Opus-4.6, and GPT-5.2. Our results show that these models generally maintain strong performance under several perturbations; however, notable performance degradation is observed for surface-level noise (e.g., character-level corruption) and linguistic variation that preserves semantics while altering lexical or syntactic forms. Furthermore, we observe that surface-level noise causes larger performance drops in traditional pipelines, whereas linguistic variation presents greater challenges in agentic settings. These findings highlight the remaining challenges in achieving robust NL2SQL systems, particularly in handling linguistic variability.

==> related.tex <==
\section{Related Work}

Several prior studies have explored the robustness and generalization capabilities of Natural Language to SQL (NL2SQL) systems. Dr.Spider~\citep{chang2023dr} extends the Spider benchmark by introducing multiple perturbations, such as linguistic variations and noise injection, to systematically evaluate model robustness under distribution shifts. Another line of work focuses on linguistic robustness. \citet{safarzadeh-etal-2025-evaluating} leverage SQL-to-NL generation to produce schema-aligned paraphrases of queries, enabling evaluation of NL2SQL models under semantically equivalent but linguistically diverse inputs. These studies highlight that previous models remain sensitive to input perturbations in traditional settings. In our work, we conduct empirical evaluations of several state-of-the-art models under both traditional and agentic settings.

